Network Inference from a Mixture of Diffusion Models for Fake News Mitigation

The dissemination of fake news intended to deceive people, influence public opinion and manipulate social outcomes, has become a pressing problem on social media. Moreover, information sharing on social media facilitates diffusion of viral information cascades. In this work, we focus on understanding and leveraging diffusion dynamics of false and legitimate contents in order to facilitate network interventions for fake news mitigation. We analyze real-world Twitter datasets comprising fake and true news cascades, to understand differences in diffusion dynamics and user behaviours with regards to fake and true contents. Based on the analysis, we model the diffusion as a mixture of Independent Cascade models (MIC) with parameters $\theta_T, \theta_F$ over the social network graph; and derive unsupervised inference techniques for parameter estimation of the diffusion mixture model from observed, unlabeled cascades. Users influential in the propagation of true and fake contents are identified using the inferred diffusion dynamics. Characteristics of the identified influential users reveal positive correlation between influential users identified for fake news and their relative appearance in fake news cascades. Identified influential users tend to be related to topics of more viral information cascades than less viral ones; and identified fake news influential users have relatively fewer counts of direct followers, compared to the true news influential users. Intervention analysis on nodes and edges demonstrates capacity of the inferred diffusion dynamics in supporting network interventions for mitigation.

==> edge.tex <==

EDGE INFL

% This can be an attribute of the data collection periods of the two datasets. Twitter-1 is collected between 2006-2009 whereas Twitter-2 is collected in 2015, and an increase in sophistication of fake content creation and social media usage could be responsible for more users encountering or engaging with both fake and true contents \cite{sharma2019combating}.

% Also, fake influential users tend to appear in both true and fake cascades more than true influential users who tend to appear in true cascades only. This could be explained by the fact that fake new spreader try to avoid detection by interacting with both types of news, an observation also made in \cite{ruchansky2017csi}.

% \begin{comment}

% \begin{figure}[t]
% \centering
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/fakeseeds_fakediffkwon1.pdf}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/fakeseeds_fakediffkwon2.pdf}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/fakeseeds_fakediffkwon3.pdf}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/fakeseeds_fakediffkwon4.pdf}
%     \end{subfigure}
%     ~
    
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/fakeseeds_truediffkwon1.pdf}
%      \caption*{Seeds (A)}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/fakeseeds_truediffkwon2.pdf}
%      \caption*{Seeds (B)}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/fakeseeds_truediffkwon3.pdf}
%      \caption*{Seeds (C)}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/fakeseeds_truediffkwon4.pdf}
%      \caption*{Seeds (D)}
%     \end{subfigure}
%     ~
% \caption{Edge influence analysis Twitter-1. Simulated cascades from seed sets (A-D) sampled from inferred influential users (true news) under (top row) $\theta_T$ and (bottom row) $\theta_F$.}
% \label{fig:sim1}
% \end{figure}

% \begin{figure}[t]
% \centering

%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/trueseeds_truediffkwon3.pdf}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/trueseeds_truediffkwon6.pdf}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/trueseeds_truediffkwon8.pdf}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/trueseeds_truediffkwon9.pdf}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/trueseeds_fakediffkwon3.pdf}
%      \caption*{Seeds (A)}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/trueseeds_fakediffkwon6.pdf}
%      \caption*{Seeds (B)}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/trueseeds_fakediffkwon8.pdf}
%      \caption*{Seeds (C)}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\columnwidth}
%      \includegraphics[width=\columnwidth]{plots/pred_cas/trueseeds_fakediffkwon9.pdf}
%      \caption*{Seeds (D)}
%     \end{subfigure}
% \caption{Edge influence analysis Twitter-1. Simulated cascades from seed sets (A-D) sampled from inferred influential users (fake news) under (top row) $\theta_F$ and (bottom row) $\theta_T$.}
% \label{fig:sim2}
% \end{figure}


% \subsection{Edge Influence Analysis} The statistical diffusion analysis earlier indicated that the influence between users is non-homogeneous with respect to fake and true cascades. In Fig~\ref{fig:sim1} and \ref{fig:sim2} we examine whether the proposed method learns differentiated edge influence parameters for the two components $\theta_T$ and $\theta_F$. In Fig~\ref{fig:sim1}, seed sets (A-D) are sampled from inferred influential users for true news. For each seed set, we simulate the diffusion model first under $\hat{\theta}_T$ (top row) and then $\hat{\theta}_F$ (bottom row). The expected cascade i.e. expected \# tweets at each time step, is obtained over 1000 simulations per seed set and plot in the figure along with its standard deviation at each time step. Similarly for inferred fake influential users in Fig~\ref{fig:sim2}.

% \noindent \textbf{Result:}  In addition, in Twitter-1 simulated cascades from true influential under $\hat{\theta}_F$ are negligible, but from fake influential under $\hat{\theta}_T$ are small but non-negligible, reflecting a likely effort from fake influential users  to  appear  reliable  through  engagements  with  both types of contents.

% We examine whether the inferred parameters To gain an insight about the learned diffusion parameters $\theta_T$ and $\theta_F$, simulated cascades from seed sets sampled uniformly from (fake and true) influential users (as identified in \ref{sec:influsers}), under both components of the diffusion mixture model are shown in Fig~\ref{fig:sim1} and \ref{fig:sim2}. 

% \end{comment}



TRAIN TIME



% \begin{figure}
%     ~
%     \begin{subfigure}[t]{0.3\columnwidth}
%     \centering
%      \includegraphics[height=2.3cm,width=\columnwidth]{plots/newtwitter_ma_train_time.png}
%     \caption{Train time:T2}
%     \label{fig:tr-time-l}
%     \end{subfigure}
% \caption{Interventions (Edge) and Training time on Twitter-1 (T1) and Twitter-2 (T2).}
% \label{fig:inter-trtime}
% \end{figure}

% Lastly, in Fig~\ref{fig:tr-time-l}, we compare the training time of the inference method MIC against SEIZ at different graph size i.e number of users varied from 1K to 10K. SEIZ training time grows rapidly as it fits diffusion parameters to each cascade separately. MIC is more scalable as the optimization with EM converges in about 8-10 iterations and the M-step has an analytical solution to solve the optimization problem to update edge parameters.


CONVERGENCE, AUC



SYNTHETIC

==> file_proof.tex <==




==> file_synexp.tex <==

In this section, we present experimental analysis on synthetic and real Twitter datasets using the proposed EM algorithm for inferring MIC parameters $\pi$, $\theta_F$, and $\theta_T$. We evaluate the quality of the inferred diffusion parameters based on their ability to separate (cluster) fake and true cascades based on the learned diffusion dynamics, and generate meaningful representations of the observed propagation dynamics. Further, we explore applications of the inferred parameters in predicting cascade dynamics and providing interventions for fake news mitigation.

\section{Synthetic datasets}\label{sec:synthetic}

We first examine the effect of varying mixture distributions on parameter estimation using the proposed algorithm on synthetic data. We construct three three sets of observed cascades at different mixture distributions $\pi$ i.e. $(0.5, 0.5)$, $(0.2, 0.8)$  and $(0.35, 0.65)$. We generate a random graph with 512 nodes and 1024 edges, and for each edge we draw the edge influence strengths uniformly between [0,1]. To generate cascades, we sample seed sets uniformly from the nodes with sizes drawn from a power law distribution with exponent $2.5$. The resulting average size of a cascade is $300$ and we vary sample size (number of cascades) from 100 to 5K.

\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{plots/newrec.png}
    \caption{\emph{Parameter Recoverability.} Mean absolute error results on estimated diffusion mixture model (MIC) parameters; variation with \# of cascades at different mixture distributions.}
 \label{fig:paramrec}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{plots/newsep.png}
  \caption{\emph{Cascade Separability.} Clustering accuracy and f1 results with estimated diffusion mixture model (MIC); variation with \# of cascades at different mixture distributions.}
 \label{fig:cassep}
\end{figure}



% \begin{figure}[t]
% \centering
%     \begin{subfigure}[t]{0.3\columnwidth}
%     \centering
%     \includegraphics[scale=0.4]{plots/newrec_5050.png}
%     \caption{Mixture (50-50)}
%     \label{nonlinear_a}
%     \end{subfigure}
% \hspace*{\fill}
%     \begin{subfigure}[t]{0.3\columnwidth}
%     \centering
%     \includegraphics[scale=0.4]{plots/newrec_2080.png}
%     \caption{Mixture (20-80)}
%     \label{nonlinear_b}
%     \end{subfigure}
% \hspace*{\fill}
%     \begin{subfigure}[t]{0.3\columnwidth}
%     \centering
%     \includegraphics[scale=0.4]{plots/newrec_3565.png}
%     \caption{Mixture (35-65)}
%     \label{nonlinear_b}
%     \end{subfigure}
% \caption{\emph{Parameter Recoverability.} Mean absolute error results on estimated diffusion mixture model (MIC) parameters; variation with \# of cascades at different mixture distributions.}
%  \label{fig:paramrec}
% \end{figure}

\subsection{Parameter recoverability and clustering cascades}
We use mean absolute error (MAE) as the metric for evaluating parameter recoverability for the mixture model, averaged over $10$ runs of the method. The inferred parameters are compared to the available ground truth values of edge influence parameters and mixing weights, for each of the two components. The results are shown in Figure \ref{fig:paramrec} below. The algorithm is able to recover parameters of both components and the mixing weights $\pi$ even with unlabeled cascades. With increase in sample size, the estimation error of mixing weights $\pi$ 
is equally good at all mixture distributions; and for smaller sample size, estimation is better for distributions closer to uniform. Estimation errors of parameters of each component are similar at uniform mixture distributions, but with skewed distributions, estimation error of the smaller component increases due to lower effective sample size.

% \subsection{Cascade separability}
% \begin{figure}[t]
% \centering
%     \begin{subfigure}[t]{0.30\columnwidth}
%     \centering
%     \includegraphics[scale=0.4]{plots/newsep_5050.png}
%     \caption{Mixture (50-50)}
%     \label{nonlinear_a}
%     \end{subfigure}
% \hspace*{\fill}
%     \begin{subfigure}[t]{0.30\columnwidth}
%     \centering
%     \includegraphics[scale=0.4]{plots/newsep_2080.png}
%     \caption{Mixture (20-80)}
%     \label{nonlinear_b}
%     \end{subfigure}
% \hspace*{\fill}
%     \begin{subfigure}[t]{0.30\columnwidth}
%     \centering
%     \includegraphics[scale=0.4]{plots/newsep_3565.png}
%     \caption{Mixture (35-65)}
%     \label{nonlinear_b}
%     \end{subfigure}
% \caption{\emph{Cascade Separability.} Clustering accuracy and f1 results with estimated diffusion mixture model (MIC); variation with \# of cascades at different mixture distributions.}
%  \label{fig:cassep}
% \end{figure}
We examine how well the cascades from the two components can be separated based on their observed diffusion patterns; in terms of clustering accuracy and f1-score metrics for each synthetic cascades set at different mixture distributions, in Figure \ref{fig:cassep}. We run the parameter estimation to infer the diffusion parameters, and calculate the posterior probability for each cascade $s \in C$ given the inferred parameter values under each component of MIC. The membership of each cascade to one of the two components is determined as $\argmax_M \gamma_s^M$, where $\gamma_s^M$ is defined Equation \ref{eqn:gamma}. Since the clustering is unsupervised, to determine which cluster corresponds to which component, we select a random stratified $20\%$ of the cascades and use their labels for determining the mapping from clusters to components. As the diffusion model parameter estimates improve with sample size, we see a corresponding improvement in the accuracy and f1-scores on clustering (separability) of the two components under the inferred parameters. Similarly, the separability of the two components is higher for mixture distributions closer to uniform as more cascades are assigned to their correct clusters from both components.


==> reviewer_response.tex <==
\begin{document}

We thank the reviewers for their response.

\begin{table}[t]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
\end{document}
